Behavior-Tree-Based Person Search for Symbiotic Autonomous Mobile Robot Tasks

We consider the problem of people search by a mobile social robot in case of a situation that cannot be solved by the robot alone. Examples are physically opening a closed door or operating an elevator. Based on the Behavior Tree framework, we create a modular and easily extendable action sequence with the goal of finding a person to assist the robot. By decomposing the Behavior Tree as a Discrete Time Markov Chain, we obtain an estimate of the probability and rate of success of the options for action, especially where the robot should wait or search for people.In a real-world experiment, the presented method is compared with other common approaches in a total of 588 test runs over the course of one week, starting at two different locations in a university building. We show our method to be superior to other approaches in terms of success rate and duration until a finding person and returning to the start location.

==> table/place_1.tex <==
\begin{tabular}{rrrrrr}
\rule{0pt}{2.5ex}Location & Method & $n_{\mathrm{trials}}$ & Success rate & $\bar{t}_\mathrm{s}$ (in \SI{}{\second}) & $\sigma_{t,\mathrm{s}}$ (in \SI{}{\second}) \\ 
\hline 
 \rule{0pt}{2.5ex}$\mathcal{P}_{\mathrm{stor}}$ & PSBT & $86$ & \SI{98.84}{\percent} & $120.49$ & $61.20$ \\ 
 & GM & $86$ & \SI{62.79}{\percent} & $101.13$ & $22.43$ \\ 
 & NW & $47$ & \SI{91.49}{\percent} & $123.04$ & $52.00$ \\ 
 & GC & $59$ & \SI{59.32}{\percent} & $93.53$ & $51.62$ \\ 
 & W & $31$ & \SI{61.29}{\percent} & $160.18$ & $133.73$ \\
 \hline\rule{0pt}{2.5ex}$\mathcal{P}_{\mathrm{cafe}}$ & PSBT & $112$ & \SI{91.07}{\percent} & $35.51$ & $28.15$ \\ 
 & NW & $85$ & \SI{91.76}{\percent} & $63.67$ & $46.67$ \\ 
\hline 
\end{tabular}

==> table/place_2.tex <==
\begin{tabular}{rrrrr}
\rule{0pt}{2.5ex}Method & $n_{\mathrm{trials}}$ & Success rate & $\bar{t}_\mathrm{s}$ (in \SI{}{\second}) & $\sigma_{t,\mathrm{s}}$ (in \SI{}{\second}) \\ 
\hline 
 \rule{0pt}{2.5ex}PSBT & $112$ & \SI{91.07}{\percent} & $35.51$ & $28.15$ \\ 
NW & $85$ & \SI{91.76}{\percent} & $63.67$ & $46.67$ \\ 
\hline 
\end{tabular}
